Automatic Testing and Validation of Level of Detail Reductions Through Supervised Learning

Modern video games are rapidly growing in size and scale, and to create rich and interesting environments, a large amount of content is needed. As a consequence, often several thousands of detailed 3D assets are used to create a single scene. As each asset's polygon mesh can contain millions of polygons, the number of polygons that need to be drawn every frame may exceed several billions. Therefore, the computational resources often limit how many detailed objects that can be displayed in a scene. To push this limit and to optimize performance one can reduce the polygon count of the assets when possible. Basically, the idea is that an object at farther distance from the capturing camera, consequently with relatively smaller screen size, its polygon count may be reduced without affecting the perceived quality. Level of Detail (LOD) refers to the complexity level of a 3D model representation. The process of removing complexity is often called LOD reduction and can be done automatically with an algorithm or by hand by artists. However, this process may lead to deterioration of the visual quality if the different LODs differ significantly, or if LOD reduction transition is not seamless. Today the validation of these results is mainly done manually requiring an expert to visually inspect the results. However, this process is slow, mundane, and therefore prone to error. Herein we propose a method to automate this process based on the use of deep convolutional networks. We report promising results and envision that this method can be used to automate the process of LOD reduction testing and validation.

==> results_old.tex <==
\section{Results}
\label{sec:results}

\subsection{Binary classification}
The first use case of this approach is binary classification, or detection of LOD transitions. The goal is to train a model which can visually inspect LOD transitions and tag either "bad" transitions or determine at which distance the transition is not visible, or at least not visibly affecting the perceived quality. The two use cases we envision for this approach are:
\begin{itemize}
\item detecting of bad transitions, e.g. when one has to parse a big asset database this could be an automatic way of classifying good and bad transitions thus helping with the process of improving large chunks of data.
\item scene optimization: instead of manually setting the distance where LOD transitions should occur, this is an automated approach where full scene could automatically be optimized to both look visually pleasing, while keeping the computational cost for polygons to a minimum. 
\end{itemize}

It figure \ref{fig:train_accuracy} and \ref{fig:validation_accuracy} we compare different selection of popular and state-of-the-art deep neural nets and their performance on this task. 

\subsubsection{Selecting CNN and hyperparameters for experiments}
In Table \ref{tab:all_nets_acc} we see that the accuracy is very high for all the networks. There weren't big differences in the accuracies so we looked a bit into the complexity of the CNN architectures and the time it took to train. Furthermore we had used the resnet networks when implementing the concatenation methods. Therefore we went ahead with testing using resnet18. The choice was made to continue with resnet18 of its complexity and because we had tested the concatenation methods using resnet18, so we knew they worked together. However, if mobilenet\_v3\_small or mobilenet\_v3\_large would've been used instead the expectation of the results would be similar to resnet18.

\begin{table}[!htb]
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
  Network & Mean Accuracy \\ 
   \hline\hline
  resnet18 & 0.995 \\ 
  resnet34 & 0.988 \\ 
  resnet50 & 0.994  \\ 
  resnet101 & 0.994  \\ 
  vgg11 & 0.985  \\ 
  vgg13 & 0.995  \\ 
  vgg16 & 0.996  \\ 
  vgg19 & 0.995  \\ 
  mobilenet\_v2 & 0.992  \\ 
  mobilenet\_v3\_large & 0.990  \\ 
  mobilenet\_v3\_small & 0.990  \\ 
 \hline
\end{tabular}
\end{center}\caption{Mean validation accuracies of the networks trained}
\end{table}\label{tab:all_nets_acc}

%The train accuracy for using each learning rate and multiple batch sizes are presented in Figure \ref{fig:lr_and_batch_01}, Figure \ref{fig:lr_and_batch_001} and Figure \ref{fig:lr_and_batch_0001}. 

%The mean validation accuracies for each learning rate are displayed in \ref{tab:lr_b_mean_val_acc}. From the graphs we can conclude that using a learning rate of 0.01 reaches an accuracy of 0.95 for all batch sizes after 2 epochs. Comparing the best combinations, we have a learning rate of 0.001 and batch size 8, a learning rate of 0.01 and batch size 32 or 64, and a learning rate of 0.1 and a batch size of 128. The ranges training times can be seen in \ref{tab:lr_b_train_time} where it seems that a smaller batch size leads to a longer training time regardless of the learning rate. It can be noticed that there is not much difference in training times between the learning rates. Since the best validation accuracy were achieved using learning rate 0.01, regardless of batch size, and the training times were similar to all tests, a learning rate of 0.01 is recommended and what we continued to test with. 

%Assuming a best learning rate of 0.01 then to choose the batch size we noticed that there seems like a pattern of a higher validation accuracy using a smaller batch size than a larger batch size. However, because the training time also increases as the batch size is smaller we decided to not make a decision right away about which batch size to use but instead we continued the testing with both batch sizes 8 and 32. 

\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
 \hline
  Batch Size & 0.1 & 0.01 & 0.001 \\ 
   \hline
  8 & 0.87 & 0.99 & 0.96\\ 
  16 & 0.86 & 0.99 & 0.96 \\ 
  32 & 0.90 & 0.98 & 0.95\\ 
  64 & 0.88 & 0.98 & 0.94\\ 
  128 & 0.91 & 0.97 & 0.90\\ 
 \hline
\end{tabular}
\end{center}\caption{The mean validation accuracy of testing the different batch sizes and learning rates.}
\label{tab:lr_b_mean_val_acc}
\end{table}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/binary/14-01_all-networks_5-fold_stacked_data-v6/14-01-2022_0113_train_accuracy.png}
    \caption{Training accuracy for binary classification.}
    \label{fig:train_accuracy}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/binary/14-01_all-networks_5-fold_stacked_data-v6/14-01-2022_0113_val_accuracy.png}
    \caption{Validation accuracy for binary classification in 10 epochs.}
    \label{fig:validation_accuracy}
\end{figure}

\subsubsection{Generalization across different asset classes}


\begin{table}[!t]
\scalebox{0.7}{
\begin{tabular}{l|llllll}
Dataset & Large pines & Small pines & Stump & Tree dead & Wood log & Wood log 2 \\ \hline
20 stones assets        & 0.91        & 0.93        & 0.94  & 0.78      & 0.84     & 0.50       \\
35 stones assets        & 0.70        & 0.91        & 0.62  & 0.75      & 0.62     & 0.97       \\
50 stones assets        & 0.70        & 0.85        & 0.59  & 0.59      & 0.50     & 0.88       \\
65 stones assets        & 0.77        & 0.89        & 0.56  & 0.59      & 0.59     & 0.78       \\
Bush \& rock  assets    & 1.00       & 1.00  & 0.81      & 0.88     & 0.72     & 1.00 \\
%Bush, rock, flowers assets      & 0.92           & 0.93           & 0.50  & 0.53      & 0.56     & 1.00     
\end{tabular}
}
\caption{Test accuracy results of different types of assets with binary classification. Training parameters: Resnet18, using 5-fold, the channels concatenation method, batch size of 8, 10 epochs, a  learning rate of 0.01 and the SGD optimiser.}
\label{tab:test_acc_results_diff_datasets}
\end{table}

In game production often new asset classes (i.e. stones, trees, bushes, etc. counts as different asset classes) will be added throughout the lifetime of the project. To evaluate the necessary amount of data require to do meaningful generalization over different asset classes, so that this algorithm can be used for new, previous unseen asset classes, we studied the change in classification rate for different sized datasets. The results in Table \ref{tab:test_acc_results_diff_datasets} shows the accuracy results for the final test set for models trained with various amount of stone assets, and model trained with both bush and rock assets.  As one might expect, just training on one asset class tend to lead to overfitting to that class, and at 65 different stones the generalization ability is significantly reduces. We can see that for the data set with only stones, increasing the amount of stone assets decreases the overall accuracy result since the model seams to be overfitted on stones and therefore have a hard time generalizing. Just by adding even just one class more, albeit similar in structure to the assets in test data, will give a significant boost in generalization on "vegetative" assets. Still it struggles with new visual structures (in this case wood, which is not present in rocks and bushes).

\subsection{Multiclass classification - Quality}
The second use case is multiclass verification which is a more demanding problem for the model as it has to learn to distinguish between different levels of LOD reductions. The goal is to see if the model can distinguish between different quality LODs and their transitions. Input is therefore one LOD0 image (original) and one LOD with lower quality. There are 6 quality levels measured in number of polygons where "0" is original and the different classes of LOD reduction depends on the original assets' vertices count. The LOD reduction steps can be seen in Table \ref{tab:quality_lvls}. Here we let class 1 represent the highest quality of reduced LOD. Each reduction is relative to the asset's original vertices count, i.e. an asset with original vertices count of 5500 reduced to quality level 4 would be reduced to 5500*0,075. The steps were chosen with regards to the number of polygons of the assets that are present in our data sets in which most assets have a vertices count less than 500 and some a count larger than 5000.


\begin{table}
\begin{center}
\begin{tabular}{|c|c c c c|} 
 \hline
  & \multicolumn{4}{ c |}{Vertices Count}  \\ [0.5ex] 
 \hline
 Quality Level & $<100$ & $<300$ & $<500$ & $>=500$ \\ 
 \hline
 1 & 0,98 & 0,9 & 0,9 & 0,5 \\ 
 \hline
 2 & 0,92 & 0,81 & 0,72 & 0,25 \\
 \hline
 3 & 0,87 & 0,73 & 0,5 & 0,13 \\
 \hline
 4 & 0,81 & 0,58 & 0,3 & 0,075 \\
 \hline
 5 & 0,76 & 0,47 & 0,15 & 0,045 \\
 \hline
 6 & 0,7 & 0,37 & 0,075 & 0,027 \\ [1ex] 
 \hline
\end{tabular}
\end{center}\caption{The quality reduction used for each quality level based on the vertices count of the asset.}
\end{table}\label{tab:quality_lvls}


As seen in the Figure \ref{fig:multiclass_confusion_matrix_val}, the model tends to confuse classification of adjacent quality classes – for example confusing quality class 2 for a class 1 or 3. We can also see that this misclassification is gradual in the sense that class 1 is misclassified as class 2 more times than it is misclassified as class 3. Therefore, the overall accuracy rate is rather low. However, these results are acceptable as similar results would be expected if a human would attempt to classify the transitions since the difference between adjacent classes is relatively small. Furthermore, because the end goal of the classification is to determine whether a LOD transition is good enough to pass, or needs to be modified, the threshold between the groups would be done through grouping for example class 1-3 to pass and 4-6 to be modified. Thus it doesn't make a difference if the model mixes up class 1 and 2.

The final tests were run using Resnet18, using 5-fold, the channels concatenation method, batch size of 8, 100 epochs, a  learning rate of 0.01 and the SGD optimiser.


\begin{figure}[!t]
    \centering
\includegraphics[width=0.4\textwidth]{Figures/multiclass/25-01_resnet18_5-fold_channels_batchsize-8_quality_data_v5_six_quality/25-01-2022_1139_train_accuracy.png}
    \includegraphics[width=0.4\textwidth]{Figures/multiclass/25-01_resnet18_5-fold_channels_batchsize-8_quality_data_v5_six_quality/25-01-2022_1139_val_accuracy.png}
    \caption{Train and validation accuracy for multiclass.}
    \label{fig:accuracy_multiclass}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/multiclass/25-01_resnet18_5-fold_channels_batchsize-8_quality_data_v5_six_quality/25-01-2022_1139_heatmap_val.png}
    \caption{Confusion matrix for validation set}
    \label{fig:multiclass_confusion_matrix_val}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/multiclass/25-01_resnet18_5-fold_channels_batchsize-8_quality_data_v5_six_quality/25-01-2022_1343_test_heatmap.png}
    \caption{Confusion matrix for final test set}
    \label{fig:multiclass_confusion_matrix_test}
\end{figure}

To compare with the binary classification we merged the classes 1-3 and 4-6 to be able to compare quantitatively, assuming the respective ground corresponds to bad vs. good transition. The accuracy is 80\%. The significant value is lower than in the case of binary classification (approx. 98\%). However, we see that most of the misclassifications happens in the neighbor classes and excluding classes 3 and 4 (they are somewhat ambiguous as the level of quality of a specific polygon count ratio is not linear) the accuracy is 94.8\%, i.e. much closer to that of the binary case and can explain some of the disparity.

Additionally, one final test was done on a test data set with never before seen assets for the model, the results can be seen in  Figure \ref{fig:multiclass_confusion_matrix_test}. The same merging of classes was done here as for the validation results above, which resulted in 0.74\% accuracy.
